A Collection of Deep Learning-based Feature-Free Approaches for Characterizing Single-Objective Continuous Fitness Landscapes

Exploratory Landscape Analysis is a powerful technique for numerically characterizing landscapes of single-objective continuous optimization problems. Landscape insights are crucial both for problem understanding as well as for assessing benchmark set diversity and composition. Despite the irrefutable usefulness of these features, they suffer from their own ailments and downsides. Hence, in this work we provide a collection of different approaches to characterize optimization landscapes. Similar to conventional landscape features, we require a small initial sample. However, instead of computing features based on that sample, we develop alternative representations of the original sample. These range from point clouds to 2D images and, therefore, are entirely feature-free. We demonstrate and validate our devised methods on the BBOB testbed and predict, with the help of Deep Learning, the high-level, expert-based landscape properties such as the degree of multimodality and the existence of funnel structures. The quality of our approaches is on par with methods relying on the traditional landscape features. Thereby, we provide an exciting new perspective on every research area which utilizes problem information such as problem understanding and algorithm design as well as automated algorithm configuration and selection.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tables/bbob-functions-reduced.tex <==
\tiny
\begin{tabular}{c||ccccc|cccc|ccccc|ccccc|ccccc}    
	\toprule
    {\bf BBOB Function} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 \\
    \midrule
    {\bf Multimodality} & none & none & high & high & none & none & none & low & low & none & none & none & none & none & high & high & high & high & high & med. & med. & low & high & high\\
    {\bf Global Structure} & none & none & strong & strong & none & none & none & none & none & none & none & none & none & none & strong & med. & med. & med. & strong & deceptive & none & none & none & weak\\
    {\bf Funnel Structure} & yes & yes & yes & yes & yes & yes & yes & yes & yes & yes & yes & yes & yes & yes & yes & none & yes & yes & yes & yes & none & none & none & yes\\
    \midrule
\end{tabular}

==> tables/bbob-functions.tex <==
\small
\begin{tabular}{@{}lllllllll@{}}
	\toprule
	{\bf BBOB Function} & {\bf Multim.} & {\bf Global Str.} & {\bf Separab.} & {\bf Var. Sc.} & {\bf Search Sp.} & {\bf Basin Size} & {\bf Gl.-Loc.} & {\bf Funnel}\\\midrule
    1: Sphere & none & none & high & none & high & none & none & yes \\
    2: Ellipsoidal separable & none & none & high & high & high & none & none & yes  \\
    3: Rastrigin separable & high & strong & high & low & high & low & yes & yes \\
    4: B\"uche-Rastrigin & high & strong & high & low & high & med. & yes & yes \\
    5: Linear Slope & none & none & high & none & high & none & none & yes \\ \midrule
    6: Attractive Sector & none & none & none & low & med. & none & none & yes \\
    7: Step Ellipsoidal & none & none & none & low & high & none & none & yes  \\
    8: Rosenbrock & low & none & none & none & med. & low & yes & yes\\
    9: Rosenbrock rotated & low & none & none & none & med. & low & yes & yes\\ \midrule
    10: Ellipsoidal high conditioned & none & none & none & high & high & none & none & yes \\
    11: Discus & none & none & none & high & high & none & none & yes\\
    12: Bent Cigar & none & none & none & high & high & none & none & yes\\
    13: Sharp Ridge & none & none & none & low & med. & none & none  & yes\\
    14: Different Powers & none & none & none & low & med. & none & none & yes\\ \midrule
    15: Rastrigin multimodal & high & strong & none & low & high & low & yes & yes\\
    16: Weierstrass & high & med. & none & med. & high & med. & yes & none\\
    17: Schaffer F7 & high & med. & none & low & med. & med. & yes & yes\\
    18: Schaffer F7 moderately ill-cond. & high & med. & none & high & med. & med. & yes & yes\\
    19: Griewank-Rosenbrock & high & strong & none & none & high & low & yes & yes\\ \midrule
    20: Schwefel & med. & deceptive & none & none & high & low & yes & yes\\
    21: Gallagher 101 Peaks & med. & none & none & med. & high & med. & yes & none\\
    22: Gallagher 21 Peaks & low & none & none & med. & high & med. & yes & none\\
    23: Katsuura & high & none & none & none & high & low & yes & none\\
    24: Lunacek bi-Rastrigin & high & weak & none & low & high & low & yes & yes\\\midrule
\end{tabular}

==> tables/model_performance_old.tex <==
\begin{tabular}{ll|c|cccc|cccc}
  \hline
Highlevel Property & Dimension & Binary Relevance & PCA & PCA-Func & MC & rMC & Transformer (k3, p100) & Transformer (k3, p500) & Transformer (k5, p100) & Transformer (k5, p500) \\ 
  \hline
\multirow{3}{*}{Multi-Modality} & 2 & \cellcolor{gray!20}0.9973 & 0.9939 & 0.9933 & 0.9738 & 0.9714 & 0.9908 & 0.9971 & 0.9803 & 0.9942 \\ 
   & 3 & \cellcolor{gray!20}0.9973 & 0.9603 & 0.9574 & 0.9583 & 0.9540 & 0.9876 & 0.9939 & 0.9709 & 0.9919 \\ 
   & 5 & 0.9989 & 0.8970 & 0.8979 & 0.9602 & 0.9472 & 0.9908 & \cellcolor{gray!20}0.9991 & 0.9883 & 0.9984 \\ 
   & 10 & \cellcolor{gray!20}0.9996 & 0.8386 & 0.8378 & 0.9529 & 0.9522 & 0.9741 & 0.9909 & 0.9694 & 0.9880 \\ 
   \midrule\multirow{3}{*}{Global Structure} & 2 & 0.9969 & 0.9925 & 0.9921 & 0.9579 & 0.9649 & 0.9913 & \cellcolor{gray!20}0.9979 & 0.9811 & 0.9931 \\ 
   & 3 & \cellcolor{gray!20}0.9963 & 0.9515 & 0.9564 & 0.9126 & 0.8985 & 0.9857 & 0.9936 & 0.9660 & 0.9892 \\ 
   & 5 & \cellcolor{gray!20}0.9976 & 0.8067 & 0.8067 & 0.8898 & 0.8586 & 0.9784 & 0.9951 & 0.9736 & 0.9944 \\ 
   & 10 & \cellcolor{gray!20}0.9990 & 0.7737 & 0.7672 & 0.9081 & 0.9112 & 0.9632 & 0.9845 & 0.9534 & 0.9842 \\ 
   \midrule\multirow{3}{*}{Funnel Structure} & 2 & 0.9985 & 0.9991 & 0.9997 & 0.9961 & 0.9955 & 0.9991 & \cellcolor{gray!20}1.0000 & 0.9973 & \cellcolor{gray!20}1.0000 \\ 
   & 3 & 0.9997 & 0.9964 & 0.9961 & 0.9982 & 0.9923 & \cellcolor{gray!20}1.0000 & \cellcolor{gray!20}1.0000 & \cellcolor{gray!20}1.0000 & \cellcolor{gray!20}1.0000 \\ 
   & 5 & \cellcolor{gray!20}1.0000 & 0.9902 & 0.9885 & 0.9967 & 0.9893 & \cellcolor{gray!20}1.0000 & \cellcolor{gray!20}1.0000 & 0.9991 & \cellcolor{gray!20}1.0000 \\ 
   & 10 & \cellcolor{gray!20}1.0000 & 0.9774 & 0.9737 & 0.9955 & 0.9911 & 0.9991 & \cellcolor{gray!20}1.0000 & 0.9994 & \cellcolor{gray!20}1.0000 \\ 
   \midrule \hline
\end{tabular}

==> tables/results_selected_test_com_dim.tex <==
\begin{tabular}{lrrrrrrrrr}
    \toprule
    & \multicolumn{8}{c}{multimodality} \\
    & \multicolumn{2}{c}{2d} & \multicolumn{2}{c}{3d} & \multicolumn{2}{c}{5d} & \multicolumn{2}{c}{10d} \\
    reduction & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro \\
    \midrule
    Transformer (k3, p500) & 0.9967 & 0.9971 & 0.9938 & 0.9939 & 0.9985 & 0.9991 & 0.9858 & 0.9909 \\
    Transformer (k5, p500) & 0.9947 & 0.9942 & 0.9915 & 0.9919 & 0.9977 & 0.9984 & 0.9852 & 0.9880 \\
    Transformer (k3, p100) & 0.9912 & 0.9908 & 0.9900 & 0.9876 & 0.9890 & 0.9908 & 0.9673 & 0.9741 \\
    Transformer (k5, p100) & 0.9843 & 0.9803 & 0.9777 & 0.9709 & 0.9853 & 0.9883 & 0.9610 & 0.9694 \\
    MC & 0.9747 & 0.9738 & 0.9507 & 0.9583 & 0.9437 & 0.9602 & 0.9435 & 0.9529 \\
    rMC & 0.9743 & 0.9714 & 0.9502 & 0.9540 & 0.9340 & 0.9472 & 0.9428 & 0.9522 \\
    PCA & 0.9947 & 0.9939 & 0.9665 & 0.9603 & 0.9110 & 0.8970 & 0.8592 & 0.8386 \\
    PCA-Func & 0.9940 & 0.9933 & 0.9643 & 0.9574 & 0.9123 & 0.8979 & 0.8582 & 0.8378 \\
    \midrule
    & \multicolumn{8}{c}{global\_structure} \\
    & \multicolumn{2}{c}{2d} & \multicolumn{2}{c}{3d} & \multicolumn{2}{c}{5d} & \multicolumn{2}{c}{10d} \\
    reduction & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro \\
    \midrule
    Transformer (k3, p500) & 0.9973 & 0.9979 & 0.9928 & 0.9936 & 0.9947 & 0.9951 & 0.9838 & 0.9845 \\
    Transformer (k5, p500) & 0.9950 & 0.9931 & 0.9888 & 0.9892 & 0.9945 & 0.9944 & 0.9830 & 0.9842 \\
    Transformer (k3, p100) & 0.9900 & 0.9913 & 0.9842 & 0.9857 & 0.9763 & 0.9784 & 0.9597 & 0.9632 \\
    Transformer (k5, p100) & 0.9818 & 0.9811 & 0.9657 & 0.9660 & 0.9703 & 0.9736 & 0.9502 & 0.9534 \\
    MC & 0.9585 & 0.9579 & 0.9127 & 0.9126 & 0.8913 & 0.8898 & 0.9207 & 0.9081 \\
    rMC & 0.9643 & 0.9649 & 0.9110 & 0.8985 & 0.8713 & 0.8586 & 0.9253 & 0.9112 \\
    PCA & 0.9922 & 0.9925 & 0.9557 & 0.9515 & 0.8560 & 0.8067 & 0.8370 & 0.7737 \\
    PCA-Func & 0.9917 & 0.9921 & 0.9587 & 0.9564 & 0.8563 & 0.8067 & 0.8332 & 0.7672 \\
    \midrule
    & \multicolumn{8}{c}{funnel} \\
    & \multicolumn{2}{c}{2d} & \multicolumn{2}{c}{3d} & \multicolumn{2}{c}{5d} & \multicolumn{2}{c}{10d} \\
    reduction & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro \\
    \midrule
    Transformer (k3, p500) & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
    Transformer (k5, p500) & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
    Transformer (k3, p100) & 0.9995 & 0.9991 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 0.9995 & 0.9991 \\
    Transformer (k5, p100) & 0.9985 & 0.9973 & 1.0000 & 1.0000 & 0.9995 & 0.9991 & 0.9997 & 0.9994 \\
    MC & 0.9978 & 0.9961 & 0.9990 & 0.9982 & 0.9982 & 0.9967 & 0.9975 & 0.9955 \\
    rMC & 0.9975 & 0.9955 & 0.9957 & 0.9923 & 0.9940 & 0.9893 & 0.9950 & 0.9911 \\
    PCA & 0.9995 & 0.9991 & 0.9980 & 0.9964 & 0.9945 & 0.9902 & 0.9872 & 0.9774 \\
    PCA-Func & 0.9998 & 0.9997 & 0.9978 & 0.9961 & 0.9935 & 0.9885 & 0.9850 & 0.9737 \\
    \bottomrule
\end{tabular}

==> tables/results_selected_valid_com_dim.tex <==
\begin{tabular}{lrrrrrrrrr}
    \toprule
    & \multicolumn{8}{c}{multimodality} \\
    & \multicolumn{2}{c}{2d} & \multicolumn{2}{c}{3d} & \multicolumn{2}{c}{5d} & \multicolumn{2}{c}{10d} \\
    reduction & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro \\
    \midrule
    Transformer (k3, p500) & 0.9998 & 0.9997 & 0.9947 & 0.9958 & 0.9965 & 0.9978 & 0.9858 & 0.9908 \\
    Transformer (k5, p500) & 0.9973 & 0.9981 & 0.9917 & 0.9938 & 0.9955 & 0.9972 & 0.9873 & 0.9907 \\
    Transformer (k3, p100) & 0.9958 & 0.9955 & 0.9830 & 0.9821 & 0.9877 & 0.9909 & 0.9620 & 0.9708 \\
    Transformer (k5, p100) & 0.9872 & 0.9860 & 0.9730 & 0.9687 & 0.9782 & 0.9843 & 0.9545 & 0.9632 \\
    MC & 0.9765 & 0.9760 & 0.9492 & 0.9533 & 0.9368 & 0.9559 & 0.9368 & 0.9499 \\
    rMC & 0.9798 & 0.9786 & 0.9458 & 0.9488 & 0.9292 & 0.9473 & 0.9432 & 0.9557 \\
    PCA-Func & 0.9937 & 0.9913 & 0.9708 & 0.9623 & 0.9213 & 0.9143 & 0.8497 & 0.8359 \\
    PCA & 0.9925 & 0.9903 & 0.9685 & 0.9603 & 0.9167 & 0.9084 & 0.8507 & 0.8386 \\
    \midrule
    & \multicolumn{8}{c}{global\_structure} \\
    & \multicolumn{2}{c}{2d} & \multicolumn{2}{c}{3d} & \multicolumn{2}{c}{5d} & \multicolumn{2}{c}{10d} \\
    reduction & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro \\
    \midrule
    Transformer (k3, p500) & 0.9987 & 0.9989 & 0.9938 & 0.9950 & 0.9927 & 0.9928 & 0.9828 & 0.9839 \\
    Transformer (k5, p500) & 0.9980 & 0.9985 & 0.9880 & 0.9883 & 0.9907 & 0.9912 & 0.9850 & 0.9861 \\
    Transformer (k3, p100) & 0.9952 & 0.9957 & 0.9790 & 0.9821 & 0.9742 & 0.9763 & 0.9547 & 0.9576 \\
    Transformer (k5, p100) & 0.9855 & 0.9865 & 0.9605 & 0.9656 & 0.9650 & 0.9673 & 0.9458 & 0.9464 \\
    MC & 0.9688 & 0.9678 & 0.9213 & 0.9203 & 0.9023 & 0.9022 & 0.9145 & 0.9111 \\
    rMC & 0.9718 & 0.9698 & 0.9285 & 0.9249 & 0.8775 & 0.8706 & 0.9253 & 0.9159 \\
    PCA-Func & 0.9945 & 0.9948 & 0.9660 & 0.9636 & 0.8753 & 0.8340 & 0.8262 & 0.7604 \\
    PCA & 0.9942 & 0.9949 & 0.9613 & 0.9590 & 0.8703 & 0.8277 & 0.8337 & 0.7701 \\
    \midrule
    & \multicolumn{8}{c}{funnel} \\
    & \multicolumn{2}{c}{2d} & \multicolumn{2}{c}{3d} & \multicolumn{2}{c}{5d} & \multicolumn{2}{c}{10d} \\
    reduction & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro & F1 Micro & F1 Macro \\
    \midrule
    Transformer (k3, p500) & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
    Transformer (k5, p500) & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
    Transformer (k3, p100) & 0.9995 & 0.9991 & 1.0000 & 1.0000 & 0.9998 & 0.9997 & 0.9997 & 0.9994 \\
    Transformer (k5, p100) & 0.9977 & 0.9958 & 0.9993 & 0.9988 & 0.9995 & 0.9991 & 0.9995 & 0.9991 \\
    MC & 0.9988 & 0.9979 & 0.9977 & 0.9958 & 0.9978 & 0.9961 & 0.9983 & 0.9970 \\
    rMC & 0.9970 & 0.9946 & 0.9948 & 0.9908 & 0.9968 & 0.9943 & 0.9953 & 0.9917 \\
    PCA & 0.9995 & 0.9991 & 0.9973 & 0.9952 & 0.9937 & 0.9887 & 0.9913 & 0.9846 \\
    PCA-Func & 0.9997 & 0.9994 & 0.9970 & 0.9946 & 0.9928 & 0.9873 & 0.9885 & 0.9798 \\
    \bottomrule
\end{tabular}

==> tables/shufflenet_multim_test_sep_dim.tex <==
\begin{tabular}{llrrrrr}
    \toprule
    &  &  &  Acc &  Balanced Acc &  F1 Micro &  F1 Macro \\
    dim & reduction &   loss &  \multicolumn{4}{c}{multimodality} \\
    \midrule
     2d &       PCA & 0.0211 &              98.72 &                       98.55 &                  0.9872 &                  0.9843 \\
     2d &  PCA-Func & 0.0241 &              98.62 &                       98.22 &                  0.9862 &                  0.9841 \\
     2d &      None & 0.0490 &              97.18 &                       96.81 &                  0.9718 &                  0.9692 \\
    \midrule
     3d &  PCA-Func & 0.0985 &              94.68 &                       95.50 &                  0.9468 &                  0.9375 \\
     3d &       PCA & 0.1010 &              94.95 &                       95.99 &                  0.9495 &                  0.9397 \\
     3d &        MC & 0.1163 &              93.47 &                       95.19 &                  0.9347 &                  0.9383 \\
     3d &       rMC & 0.1264 &              93.08 &                       94.81 &                  0.9308 &                  0.9328 \\
    \midrule
     5d &       rMC & 0.1045 &              93.40 &                       95.53 &                  0.9340 &                  0.9467 \\
     5d &        MC & 0.1090 &              93.17 &                       95.52 &                  0.9317 &                  0.9456 \\
     5d &  PCA-Func & 0.2555 &              87.92 &                       88.58 &                  0.8792 &                  0.8608 \\
     5d &       PCA & 0.2562 &              87.60 &                       88.54 &                  0.8760 &                  0.8571 \\
    \midrule
     10d &       rMC & 0.0894 &              94.57 &                       96.45 &                  0.9457 &                  0.9545 \\
     10d &        MC & 0.0973 &              94.33 &                       96.21 &                  0.9433 &                  0.9556 \\
     10d &  PCA-Func & 0.3535 &              82.70 &                       85.46 &                  0.8270 &                  0.8053 \\
     10d &       PCA & 0.3717 &              81.58 &                       84.62 &                  0.8158 &                  0.7960 \\
    \bottomrule
\end{tabular}

==> tables/shufflenet_multim_valid_sep_dim.tex <==
\begin{tabular}{llrrrrr}
    \toprule
      &  &  &  Acc &  Balanced Acc &  F1 Micro &  F1 Macro \\
    dim & reduction &   loss &  \multicolumn{4}{c}{multimodality} \\
    \midrule
     2d &       PCA & 0.0211 &              98.90 &                       98.93 &                  0.9890 &                  0.9869 \\
     2d &  PCA-Func & 0.0241 &              99.07 &                       99.12 &                  0.9907 &                  0.9895 \\
     2d &      None & 0.0490 &              97.88 &                       97.84 &                  0.9788 &                  0.9784 \\
    \midrule
     3d &  PCA-Func & 0.0985 &              95.97 &                       96.98 &                  0.9597 &                  0.9521 \\
     3d &       PCA & 0.1010 &              95.55 &                       96.72 &                  0.9555 &                  0.9471 \\
     3d &        MC & 0.1163 &              94.02 &                       95.39 &                  0.9402 &                  0.9415 \\
     3d &       rMC & 0.1264 &              93.73 &                       95.34 &                  0.9373 &                  0.9402 \\
    \midrule
     5d &       rMC & 0.1045 &              93.03 &                       95.37 &                  0.9303 &                  0.9464 \\
     5d &        MC & 0.1090 &              93.13 &                       95.44 &                  0.9313 &                  0.9483 \\
     5d &  PCA-Func & 0.2555 &              88.67 &                       89.47 &                  0.8867 &                  0.8740 \\
     5d &       PCA & 0.2562 &              88.42 &                       89.52 &                  0.8842 &                  0.8735 \\
    \midrule
     10d &       rMC & 0.0894 &              94.08 &                       96.16 &                  0.9408 &                  0.9548 \\
     10d &        MC & 0.0973 &              93.53 &                       95.62 &                  0.9353 &                  0.9493 \\
     10d &  PCA-Func & 0.3535 &              81.90 &                       85.49 &                  0.8190 &                  0.8067 \\
     10d &       PCA & 0.3717 &              81.37 &                       84.73 &                  0.8137 &                  0.7995 \\
    \bottomrule
\end{tabular}

==> tables/shufflenet_selected_test_sep_dim.tex <==
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
& & & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Balanced Accuracy} & \multicolumn{3}{c}{F1-Micro} & \multicolumn{3}{c}{F1-Macro} \\
dim & reduction & loss & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel \\
\midrule
 2d & PCA-Func & 0.0366 & 98.95 & 98.63 & 99.88 & 98.71 & 99.43 & 99.89 & 0.9895 & 0.9863 & 0.9988 & 0.9877 & 0.9878 & 0.9979 \\
 2d & PCA & 0.0403 & 98.85 & 98.43 & 99.95 & 98.24 & 99.41 & 99.85 & 0.9885 & 0.9843 & 0.9995 & 0.9854 & 0.9857 & 0.9991 \\
 2d & None & 0.0914 & 97.93 & 97.22 & 99.88 & 97.61 & 98.18 & 99.89 & 0.9793 & 0.9722 & 0.9988 & 0.9775 & 0.9723 & 0.9979 \\
\midrule
 3d & PCA-Func & 0.1998 & 95.32 & 94.32 & 99.70 & 96.20 & 96.15 & 99.82 & 0.9532 & 0.9432 & 0.9970 & 0.9441 & 0.9383 & 0.9946 \\
 3d & PCA & 0.2233 & 95.17 & 93.85 & 99.70 & 95.79 & 96.26 & 99.78 & 0.9517 & 0.9385 & 0.9970 & 0.9422 & 0.9321 & 0.9946 \\
 3d & rMC & 0.2963 & 93.57 & 90.63 & 99.47 & 95.30 & 92.07 & 99.64 & 0.9357 & 0.9063 & 0.9947 & 0.9395 & 0.8932 & 0.9905 \\
 3d & MC & 0.3054 & 94.67 & 91.53 & 99.65 & 96.02 & 92.36 & 99.67 & 0.9467 & 0.9153 & 0.9965 & 0.9507 & 0.9004 & 0.9937 \\
\midrule
 5d & rMC & 0.2683 & 94.25 & 88.83 & 99.55 & 96.06 & 92.61 & 99.69 & 0.9425 & 0.8883 & 0.9955 & 0.9538 & 0.8726 & 0.9920 \\
 5d & MC & 0.2776 & 93.73 & 88.18 & 99.78 & 95.79 & 92.43 & 99.87 & 0.9373 & 0.8818 & 0.9978 & 0.9531 & 0.8725 & 0.9961 \\
 5d & PCA & 0.5169 & 89.28 & 82.10 & 99.18 & 90.26 & 88.94 & 99.35 & 0.8928 & 0.8210 & 0.9918 & 0.8789 & 0.7648 & 0.9855 \\
 5d & PCA-Func & 0.5294 & 88.92 & 82.08 & 99.15 & 89.39 & 88.92 & 99.37 & 0.8892 & 0.8208 & 0.9915 & 0.8702 & 0.7646 & 0.9850 \\
\midrule
 10d & rMC & 0.2035 & 94.47 & 92.48 & 99.62 & 96.32 & 96.27 & 99.77 & 0.9447 & 0.9248 & 0.9962 & 0.9537 & 0.9115 & 0.9932 \\
 10d & MC & 0.2297 & 94.43 & 92.78 & 99.47 & 96.26 & 95.66 & 99.68 & 0.9443 & 0.9278 & 0.9947 & 0.9522 & 0.9184 & 0.9905 \\
 10d & PCA-Func & 0.7641 & 82.95 & 78.53 & 97.57 & 85.65 & 86.15 & 97.90 & 0.8295 & 0.7853 & 0.9757 & 0.8058 & 0.7153 & 0.9581 \\
 10d & PCA & 0.8309 & 82.08 & 76.75 & 97.17 & 84.42 & 84.51 & 97.42 & 0.8208 & 0.7675 & 0.9717 & 0.7978 & 0.6956 & 0.9514 \\
\bottomrule
\end{tabular}

==> tables/shufflenet_selected_valid_sep_dim.tex <==
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
& & & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Balanced Accuracy} & \multicolumn{3}{c}{F1-Micro} & \multicolumn{3}{c}{F1-Macro} \\
dim & reduction & loss & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel \\
\midrule
 2d & PCA-Func & 0.0366 & 99.17 & 99.07 & 99.95 & 99.15 & 99.41 & 99.97 & 0.9917 & 0.9907 & 0.9995 & 0.9897 & 0.9916 & 0.9991 \\
 2d & PCA & 0.0403 & 98.97 & 98.90 & 99.93 & 98.79 & 99.30 & 99.96 & 0.9897 & 0.9890 & 0.9993 & 0.9869 & 0.9901 & 0.9988 \\
 2d & None & 0.0914 & 98.50 & 98.08 & 99.85 & 98.11 & 98.28 & 99.79 & 0.9850 & 0.9808 & 0.9985 & 0.9832 & 0.9798 & 0.9973 \\
\midrule
 3d & PCA-Func & 0.1998 & 96.47 & 95.10 & 99.62 & 97.16 & 96.68 & 99.69 & 0.9647 & 0.9510 & 0.9962 & 0.9567 & 0.9494 & 0.9932 \\
 3d & PCA & 0.2233 & 95.33 & 94.18 & 99.62 & 96.15 & 96.37 & 99.61 & 0.9533 & 0.9418 & 0.9962 & 0.9443 & 0.9377 & 0.9931 \\
 3d & rMC & 0.2963 & 94.08 & 92.42 & 99.55 & 95.67 & 93.76 & 99.65 & 0.9408 & 0.9242 & 0.9955 & 0.9448 & 0.9181 & 0.9920 \\
 3d & MC & 0.3054 & 94.70 & 93.22 & 99.65 & 95.94 & 93.40 & 99.75 & 0.9470 & 0.9322 & 0.9965 & 0.9494 & 0.9244 & 0.9937 \\
\midrule
 5d & rMC & 0.2683 & 93.63 & 89.43 & 99.65 & 95.83 & 93.05 & 99.79 & 0.9363 & 0.8943 & 0.9965 & 0.9517 & 0.8816 & 0.9938 \\
 5d & MC & 0.2776 & 93.28 & 89.80 & 99.75 & 95.49 & 93.00 & 99.81 & 0.9328 & 0.8980 & 0.9975 & 0.9500 & 0.8922 & 0.9955 \\
 5d & PCA & 0.5169 & 89.10 & 83.47 & 99.15 & 89.85 & 90.48 & 99.37 & 0.8910 & 0.8347 & 0.9915 & 0.8782 & 0.7840 & 0.9850 \\
 5d & PCA-Func & 0.5294 & 89.02 & 83.43 & 99.15 & 89.67 & 90.03 & 99.29 & 0.8902 & 0.8343 & 0.9915 & 0.8770 & 0.7821 & 0.9849 \\
\midrule
 10d & rMC & 0.2035 & 94.25 & 92.43 & 99.72 & 96.26 & 95.95 & 99.79 & 0.9425 & 0.9243 & 0.9972 & 0.9547 & 0.9151 & 0.9949 \\
 10d & MC & 0.2297 & 93.65 & 92.52 & 99.72 & 95.72 & 95.48 & 99.79 & 0.9365 & 0.9252 & 0.9972 & 0.9476 & 0.9178 & 0.9949 \\
 10d & PCA-Func & 0.7641 & 81.92 & 77.78 & 97.93 & 85.74 & 86.23 & 98.40 & 0.8192 & 0.7778 & 0.9793 & 0.8061 & 0.7106 & 0.9643 \\
 10d & PCA & 0.8309 & 81.67 & 76.47 & 97.43 & 84.49 & 85.00 & 97.74 & 0.8167 & 0.7647 & 0.9743 & 0.8014 & 0.6967 & 0.9559 \\
\bottomrule
\end{tabular}

==> tables/transformer_selected_test_embedding.tex <==
\begin{tabular}{llllrrrrrrrrrrrrr}
\toprule
& & & & & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Balanced Accuracy} & \multicolumn{3}{c}{F1-Micro} & \multicolumn{3}{c}{F1-Macro} \\
dim & k & p & d & loss & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel \\
\midrule
 3d & k3 & p1.0 & d2.0 & 0.0722 & 98.88 & 98.40 & 99.98 & 99.26 & 99.05 & 99.99 & 0.9888 & 0.9840 & 0.9998 & 0.9898 & 0.9861 & 0.9997 \\
 3d & k3 & p2.0 & d2.0 & 0.0801 & 98.70 & 98.42 & 100.00 & 99.10 & 98.93 & 100.00 & 0.9870 & 0.9842 & 1.0000 & 0.9877 & 0.9863 & 1.0000 \\
 3d & k3 & p2.0 & dinf & 0.0815 & 98.92 & 98.38 & 100.00 & 99.23 & 99.01 & 100.00 & 0.9892 & 0.9838 & 1.0000 & 0.9895 & 0.9866 & 1.0000 \\
 3d & k3 & p1.0 & dinf & 0.0832 & 99.05 & 98.65 & 100.00 & 99.27 & 99.09 & 100.00 & 0.9905 & 0.9865 & 1.0000 & 0.9901 & 0.9875 & 1.0000 \\
 3d & k3 & p2.0 & d1.5 & 0.0845 & 98.75 & 98.10 & 100.00 & 99.21 & 98.74 & 100.00 & 0.9875 & 0.9810 & 1.0000 & 0.9883 & 0.9830 & 1.0000 \\
 3d & k5 & p1.0 & d1.5 & 0.0877 & 98.75 & 98.25 & 100.00 & 99.16 & 98.72 & 100.00 & 0.9875 & 0.9825 & 1.0000 & 0.9884 & 0.9841 & 1.0000 \\
 3d & k3 & pinf & d2.0 & 0.0889 & 98.60 & 97.77 & 100.00 & 99.07 & 98.65 & 100.00 & 0.9860 & 0.9777 & 1.0000 & 0.9865 & 0.9804 & 1.0000 \\
 3d & k3 & pinf & dinf & 0.0894 & 98.80 & 98.10 & 100.00 & 99.18 & 98.90 & 100.00 & 0.9880 & 0.9810 & 1.0000 & 0.9884 & 0.9825 & 1.0000 \\
 3d & k3 & p1.0 & d1.5 & 0.0914 & 98.73 & 98.22 & 100.00 & 99.08 & 98.91 & 100.00 & 0.9873 & 0.9822 & 1.0000 & 0.9875 & 0.9838 & 1.0000 \\
 3d & k3 & p2.0 & d2.5 & 0.0927 & 98.52 & 97.97 & 100.00 & 99.02 & 98.61 & 100.00 & 0.9852 & 0.9797 & 1.0000 & 0.9863 & 0.9816 & 1.0000 \\
\midrule
 5d & k3 & pinf & d1.0 & 0.0962 & 98.10 & 97.78 & 99.98 & 98.77 & 98.56 & 99.99 & 0.9810 & 0.9778 & 0.9998 & 0.9871 & 0.9796 & 0.9997 \\
 5d & k5 & p1.0 & d1.0 & 0.1096 & 98.30 & 97.10 & 99.98 & 98.93 & 98.04 & 99.99 & 0.9830 & 0.9710 & 0.9998 & 0.9889 & 0.9729 & 0.9997 \\
 5d & k5 & pinf & d1.5 & 0.1121 & 98.07 & 97.45 & 99.98 & 98.78 & 98.18 & 99.99 & 0.9807 & 0.9745 & 0.9998 & 0.9874 & 0.9767 & 0.9997 \\
 5d & k5 & pinf & d1.0 & 0.1138 & 97.62 & 97.08 & 99.97 & 98.52 & 98.21 & 99.98 & 0.9762 & 0.9708 & 0.9997 & 0.9842 & 0.9736 & 0.9994 \\
 5d & k5 & p1.0 & d2.5 & 0.1160 & 98.33 & 96.48 & 100.00 & 98.97 & 97.41 & 100.00 & 0.9833 & 0.9648 & 1.0000 & 0.9891 & 0.9635 & 1.0000 \\
 5d & k3 & pinf & dinf & 0.1282 & 97.77 & 96.73 & 99.98 & 98.61 & 97.81 & 99.99 & 0.9777 & 0.9673 & 0.9998 & 0.9853 & 0.9685 & 0.9997 \\
 5d & k3 & pinf & d1.5 & 0.1380 & 98.03 & 97.23 & 99.97 & 98.75 & 98.21 & 99.98 & 0.9803 & 0.9723 & 0.9997 & 0.9867 & 0.9740 & 0.9994 \\
 5d & k3 & p2.0 & d1.0 & 0.1441 & 97.65 & 96.67 & 99.98 & 98.45 & 98.04 & 99.99 & 0.9765 & 0.9667 & 0.9998 & 0.9841 & 0.9673 & 0.9997 \\
 5d & k3 & pinf & d2.0 & 0.1565 & 97.63 & 96.08 & 99.92 & 98.48 & 97.30 & 99.95 & 0.9763 & 0.9608 & 0.9992 & 0.9835 & 0.9621 & 0.9985 \\
 5d & k5 & p1.0 & d2.0 & 0.1657 & 97.82 & 95.25 & 100.00 & 98.63 & 96.19 & 100.00 & 0.9782 & 0.9525 & 1.0000 & 0.9853 & 0.9516 & 1.0000 \\
\midrule
10d & k5 & pinf & d1.5 & 0.1032 & 97.72 & 97.55 & 100.00 & 98.57 & 98.16 & 100.00 & 0.9772 & 0.9755 & 1.0000 & 0.9848 & 0.9760 & 1.0000 \\
10d & k3 & p2.0 & d1.0 & 0.1040 & 98.08 & 97.87 & 100.00 & 98.74 & 98.55 & 100.00 & 0.9808 & 0.9787 & 1.0000 & 0.9867 & 0.9794 & 1.0000 \\
10d & k3 & pinf & d1.5 & 0.1083 & 97.63 & 97.77 & 100.00 & 98.51 & 98.40 & 100.00 & 0.9763 & 0.9777 & 1.0000 & 0.9844 & 0.9787 & 1.0000 \\
10d & k3 & p1.0 & d1.5 & 0.1124 & 97.63 & 97.70 & 100.00 & 98.43 & 98.12 & 100.00 & 0.9763 & 0.9770 & 1.0000 & 0.9830 & 0.9769 & 1.0000 \\
10d & k5 & pinf & d2.0 & 0.1129 & 97.37 & 97.58 & 100.00 & 98.34 & 98.12 & 100.00 & 0.9737 & 0.9758 & 1.0000 & 0.9827 & 0.9773 & 1.0000 \\
10d & k3 & pinf & d1.0 & 0.1135 & 97.23 & 97.10 & 100.00 & 98.24 & 98.04 & 100.00 & 0.9723 & 0.9710 & 1.0000 & 0.9810 & 0.9711 & 1.0000 \\
10d & k3 & p2.0 & d1.5 & 0.1322 & 97.17 & 97.25 & 100.00 & 98.17 & 97.98 & 100.00 & 0.9717 & 0.9725 & 1.0000 & 0.9809 & 0.9734 & 1.0000 \\
10d & k5 & p2.0 & d1.0 & 0.1334 & 97.07 & 97.25 & 100.00 & 98.11 & 98.00 & 100.00 & 0.9707 & 0.9725 & 1.0000 & 0.9798 & 0.9742 & 1.0000 \\
10d & k5 & p1.0 & d1.5 & 0.1399 & 97.02 & 97.15 & 99.98 & 98.12 & 97.74 & 99.99 & 0.9702 & 0.9715 & 0.9998 & 0.9799 & 0.9723 & 0.9997 \\
10d & k3 & pinf & d2.5 & 0.1496 & 96.80 & 96.72 & 100.00 & 97.90 & 97.59 & 100.00 & 0.9680 & 0.9672 & 1.0000 & 0.9773 & 0.9658 & 1.0000 \\
\bottomrule
\end{tabular}

==> tables/transformer_selected_test_sep_dim.tex <==
\begin{tabular}{llllrrrrrrrrrrrrr}
\toprule
& & & & & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Balanced Accuracy} & \multicolumn{3}{c}{F1-Micro} & \multicolumn{3}{c}{F1-Macro} \\
dim & k & p & d & loss & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel \\
\midrule
 2d & k5 & p2.0 & d2.5 & 0.0239 & 98.80 & 98.72 & 99.93 & 98.68 & 99.40 & 99.96 & 0.9880 & 0.9872 & 0.9993 & 0.9866 & 0.9879 & 0.9988 \\
 2d & k5 & p2.0 & d2.0 & 0.0240 & 98.90 & 99.00 & 99.90 & 99.07 & 99.51 & 99.90 & 0.9890 & 0.9900 & 0.9990 & 0.9881 & 0.9908 & 0.9982 \\
 2d & k5 & p2.0 & dinf & 0.0254 & 98.92 & 98.75 & 99.93 & 98.99 & 99.49 & 99.92 & 0.9892 & 0.9875 & 0.9993 & 0.9868 & 0.9860 & 0.9988 \\
 2d & k5 & p1.0 & d2.5 & 0.0265 & 98.97 & 98.97 & 99.88 & 98.94 & 99.57 & 99.93 & 0.9897 & 0.9897 & 0.9988 & 0.9887 & 0.9909 & 0.9979 \\
 2d & k3 & pinf & d1.0 & 0.0268 & 99.13 & 98.92 & 99.95 & 99.07 & 99.54 & 99.97 & 0.9913 & 0.9892 & 0.9995 & 0.9905 & 0.9900 & 0.9991 \\
 2d & k3 & p1.0 & d2.5 & 0.0275 & 99.17 & 98.68 & 99.98 & 98.97 & 99.50 & 99.99 & 0.9917 & 0.9868 & 0.9998 & 0.9910 & 0.9868 & 0.9997 \\
 2d & k3 & pinf & d1.5 & 0.0284 & 99.13 & 98.93 & 99.93 & 99.00 & 99.56 & 99.96 & 0.9913 & 0.9893 & 0.9993 & 0.9912 & 0.9897 & 0.9988 \\
 2d & k3 & p2.0 & d1.5 & 0.0296 & 98.97 & 98.73 & 99.97 & 98.88 & 99.51 & 99.98 & 0.9897 & 0.9873 & 0.9997 & 0.9890 & 0.9874 & 0.9994 \\
 2d & k3 & p2.0 & d2.5 & 0.0298 & 99.00 & 98.67 & 99.98 & 98.91 & 99.41 & 99.99 & 0.9900 & 0.9867 & 0.9998 & 0.9891 & 0.9881 & 0.9997 \\
 2d & k5 & p1.0 & d2.0 & 0.0300 & 98.93 & 99.02 & 99.85 & 98.90 & 99.49 & 99.87 & 0.9893 & 0.9902 & 0.9985 & 0.9889 & 0.9913 & 0.9973 \\
 2d & k3 & pinf & d2.5 & 0.0302 & 98.88 & 98.70 & 99.93 & 98.75 & 99.41 & 99.96 & 0.9888 & 0.9870 & 0.9993 & 0.9889 & 0.9875 & 0.9988 \\
 2d & k3 & p1.0 & d2.0 & 0.0309 & 98.92 & 98.82 & 100.00 & 98.91 & 99.53 & 100.00 & 0.9892 & 0.9882 & 1.0000 & 0.9879 & 0.9880 & 1.0000 \\
 2d & k3 & pinf & dinf & 0.0309 & 99.07 & 98.68 & 99.95 & 98.91 & 99.44 & 99.97 & 0.9907 & 0.9868 & 0.9995 & 0.9904 & 0.9885 & 0.9991 \\
 2d & k3 & p2.0 & d2.0 & 0.0313 & 98.93 & 98.52 & 99.95 & 98.72 & 99.42 & 99.97 & 0.9893 & 0.9852 & 0.9995 & 0.9880 & 0.9849 & 0.9991 \\
 2d & k3 & p1.0 & d1.5 & 0.0313 & 98.98 & 98.70 & 99.93 & 98.89 & 99.39 & 99.96 & 0.9898 & 0.9870 & 0.9993 & 0.9891 & 0.9879 & 0.9988 \\
 2d & k3 & p1.0 & dinf & 0.0321 & 98.95 & 98.55 & 99.97 & 98.87 & 99.38 & 99.98 & 0.9895 & 0.9855 & 0.9997 & 0.9888 & 0.9851 & 0.9994 \\
 2d & k5 & pinf & d2.0 & 0.0321 & 98.68 & 98.62 & 99.90 & 98.56 & 99.38 & 99.90 & 0.9868 & 0.9862 & 0.9990 & 0.9860 & 0.9864 & 0.9982 \\
 2d & k5 & pinf & d2.5 & 0.0322 & 99.02 & 98.82 & 99.92 & 98.95 & 99.51 & 99.91 & 0.9902 & 0.9882 & 0.9992 & 0.9897 & 0.9869 & 0.9985 \\
 2d & k5 & p1.0 & dinf & 0.0324 & 98.85 & 98.77 & 99.88 & 98.76 & 99.45 & 99.89 & 0.9885 & 0.9877 & 0.9988 & 0.9871 & 0.9893 & 0.9979 \\
 2d & k3 & p1.0 & d1.0 & 0.0332 & 99.00 & 98.40 & 99.97 & 98.80 & 99.36 & 99.98 & 0.9900 & 0.9840 & 0.9997 & 0.9899 & 0.9845 & 0.9994 \\
\bottomrule
\end{tabular}

==> tables/transformer_selected_valid_embedding.tex <==
\begin{tabular}{llllrrrrrrrrrrrrr}
\toprule
& & & & & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Balanced Accuracy} & \multicolumn{3}{c}{F1-Micro} & \multicolumn{3}{c}{F1-Macro} \\
dim & k & p & d & loss & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel \\
\midrule
 3d & k3 & p1.0 & d2.0 & 0.0722 & 98.73 & 98.28 & 100.00 & 99.18 & 98.69 & 100.00 & 0.9873 & 0.9828 & 1.0000 & 0.9909 & 0.9845 & 1.0000 \\
 3d & k3 & p2.0 & d2.0 & 0.0801 & 98.62 & 98.13 & 100.00 & 99.10 & 98.53 & 100.00 & 0.9862 & 0.9813 & 1.0000 & 0.9904 & 0.9845 & 1.0000 \\
 3d & k3 & p2.0 & dinf & 0.0815 & 98.47 & 98.25 & 100.00 & 98.93 & 98.55 & 100.00 & 0.9847 & 0.9825 & 1.0000 & 0.9884 & 0.9853 & 1.0000 \\
 3d & k3 & p1.0 & dinf & 0.0832 & 98.60 & 98.10 & 99.98 & 99.01 & 98.64 & 99.99 & 0.9860 & 0.9810 & 0.9998 & 0.9893 & 0.9839 & 0.9997 \\
 3d & k3 & p2.0 & d1.5 & 0.0845 & 98.47 & 98.08 & 100.00 & 98.97 & 98.56 & 100.00 & 0.9847 & 0.9808 & 1.0000 & 0.9888 & 0.9832 & 1.0000 \\
 3d & k5 & p1.0 & d1.5 & 0.0877 & 98.38 & 97.95 & 100.00 & 98.92 & 98.41 & 100.00 & 0.9838 & 0.9795 & 1.0000 & 0.9878 & 0.9828 & 1.0000 \\
 3d & k3 & pinf & d2.0 & 0.0889 & 98.43 & 97.78 & 100.00 & 98.90 & 98.49 & 100.00 & 0.9843 & 0.9778 & 1.0000 & 0.9882 & 0.9811 & 1.0000 \\
 3d & k3 & pinf & dinf & 0.0894 & 98.38 & 97.85 & 100.00 & 98.78 & 98.38 & 100.00 & 0.9838 & 0.9785 & 1.0000 & 0.9871 & 0.9817 & 1.0000 \\
 3d & k3 & p1.0 & d1.5 & 0.0914 & 98.27 & 97.68 & 100.00 & 98.88 & 98.37 & 100.00 & 0.9827 & 0.9768 & 1.0000 & 0.9871 & 0.9807 & 1.0000 \\
 3d & k3 & p2.0 & d2.5 & 0.0927 & 98.42 & 97.73 & 100.00 & 98.90 & 98.50 & 100.00 & 0.9842 & 0.9773 & 1.0000 & 0.9883 & 0.9806 & 1.0000 \\
\midrule
 5d & k3 & pinf & d1.0 & 0.0962 & 97.77 & 97.57 & 99.97 & 98.56 & 97.99 & 99.98 & 0.9777 & 0.9757 & 0.9997 & 0.9857 & 0.9795 & 0.9994 \\
 5d & k5 & p1.0 & d1.0 & 0.1096 & 97.63 & 97.28 & 99.98 & 98.48 & 97.65 & 99.99 & 0.9763 & 0.9728 & 0.9998 & 0.9843 & 0.9755 & 0.9997 \\
 5d & k5 & pinf & d1.5 & 0.1121 & 97.45 & 97.00 & 99.98 & 98.34 & 97.24 & 99.99 & 0.9745 & 0.9700 & 0.9998 & 0.9837 & 0.9735 & 0.9997 \\
 5d & k5 & pinf & d1.0 & 0.1138 & 97.05 & 96.62 & 99.98 & 98.09 & 97.35 & 99.99 & 0.9705 & 0.9662 & 0.9998 & 0.9812 & 0.9707 & 0.9997 \\
 5d & k5 & p1.0 & d2.5 & 0.1160 & 97.65 & 96.62 & 100.00 & 98.51 & 97.18 & 100.00 & 0.9765 & 0.9662 & 1.0000 & 0.9848 & 0.9684 & 1.0000 \\
 5d & k3 & pinf & dinf & 0.1282 & 96.95 & 96.47 & 99.98 & 98.04 & 97.21 & 99.99 & 0.9695 & 0.9647 & 0.9998 & 0.9795 & 0.9685 & 0.9997 \\
 5d & k3 & pinf & d1.5 & 0.1380 & 97.17 & 96.63 & 99.98 & 98.16 & 97.21 & 99.99 & 0.9717 & 0.9663 & 0.9998 & 0.9817 & 0.9701 & 0.9997 \\
 5d & k3 & p2.0 & d1.0 & 0.1441 & 96.62 & 96.42 & 99.98 & 97.76 & 97.01 & 99.99 & 0.9662 & 0.9642 & 0.9998 & 0.9777 & 0.9669 & 0.9997 \\
 5d & k3 & pinf & d2.0 & 0.1565 & 96.65 & 95.83 & 99.98 & 97.85 & 96.65 & 99.99 & 0.9665 & 0.9583 & 0.9998 & 0.9776 & 0.9619 & 0.9997 \\
 5d & k5 & p1.0 & d2.0 & 0.1657 & 97.20 & 95.68 & 100.00 & 98.21 & 96.08 & 100.00 & 0.9720 & 0.9568 & 1.0000 & 0.9817 & 0.9576 & 1.0000 \\
\midrule
10d & k5 & pinf & d1.5 & 0.1032 & 97.58 & 97.25 & 100.00 & 98.47 & 97.82 & 100.00 & 0.9758 & 0.9725 & 1.0000 & 0.9837 & 0.9750 & 1.0000 \\
10d & k3 & p2.0 & d1.0 & 0.1040 & 97.97 & 97.90 & 100.00 & 98.71 & 98.43 & 100.00 & 0.9797 & 0.9790 & 1.0000 & 0.9868 & 0.9805 & 1.0000 \\
10d & k3 & pinf & d1.5 & 0.1083 & 97.88 & 97.63 & 100.00 & 98.66 & 98.22 & 100.00 & 0.9788 & 0.9763 & 1.0000 & 0.9860 & 0.9782 & 1.0000 \\
10d & k3 & p1.0 & d1.5 & 0.1124 & 97.35 & 97.00 & 100.00 & 98.31 & 97.88 & 100.00 & 0.9735 & 0.9700 & 1.0000 & 0.9815 & 0.9722 & 1.0000 \\
10d & k5 & pinf & d2.0 & 0.1129 & 97.78 & 97.45 & 100.00 & 98.59 & 97.87 & 100.00 & 0.9778 & 0.9745 & 1.0000 & 0.9852 & 0.9761 & 1.0000 \\
10d & k3 & pinf & d1.0 & 0.1135 & 97.47 & 97.27 & 100.00 & 98.35 & 98.09 & 100.00 & 0.9747 & 0.9727 & 1.0000 & 0.9822 & 0.9729 & 1.0000 \\
10d & k3 & p2.0 & d1.5 & 0.1322 & 97.23 & 96.75 & 100.00 & 98.25 & 97.44 & 100.00 & 0.9723 & 0.9675 & 1.0000 & 0.9816 & 0.9672 & 1.0000 \\
10d & k5 & p2.0 & d1.0 & 0.1334 & 97.30 & 96.97 & 100.00 & 98.24 & 97.62 & 100.00 & 0.9730 & 0.9697 & 1.0000 & 0.9816 & 0.9710 & 1.0000 \\
10d & k5 & p1.0 & d1.5 & 0.1399 & 96.58 & 96.25 & 99.98 & 97.79 & 96.96 & 99.99 & 0.9658 & 0.9625 & 0.9998 & 0.9761 & 0.9656 & 0.9997 \\
10d & k3 & pinf & d2.5 & 0.1496 & 97.08 & 96.50 & 100.00 & 98.15 & 97.47 & 100.00 & 0.9708 & 0.9650 & 1.0000 & 0.9805 & 0.9638 & 1.0000 \\
\bottomrule
\end{tabular}

==> tables/transformer_selected_valid_sep_dim.tex <==
\begin{tabular}{llllrrrrrrrrrrrrr}
\toprule
& & & & & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Balanced Accuracy} & \multicolumn{3}{c}{F1-Micro} & \multicolumn{3}{c}{F1-Macro} \\
dim & k & p & d & loss & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel & multim. & gl.\_struc. & funnel \\
\midrule
 2d & k5 & p2.0 & d2.5 & 0.0239 & 99.65 & 99.55 & 99.97 & 99.61 & 99.63 & 99.98 & 0.9965 & 0.9955 & 0.9997 & 0.9967 & 0.9962 & 0.9994 \\
 2d & k5 & p2.0 & d2.0 & 0.0240 & 99.55 & 99.47 & 99.95 & 99.53 & 99.57 & 99.93 & 0.9955 & 0.9947 & 0.9995 & 0.9954 & 0.9953 & 0.9991 \\
 2d & k5 & p2.0 & dinf & 0.0254 & 99.53 & 99.50 & 99.92 & 99.59 & 99.67 & 99.91 & 0.9953 & 0.9950 & 0.9992 & 0.9950 & 0.9958 & 0.9985 \\
 2d & k5 & p1.0 & d2.5 & 0.0265 & 99.70 & 99.58 & 99.95 & 99.68 & 99.69 & 99.97 & 0.9970 & 0.9958 & 0.9995 & 0.9968 & 0.9960 & 0.9991 \\
 2d & k3 & pinf & d1.0 & 0.0268 & 99.68 & 99.67 & 100.00 & 99.69 & 99.72 & 100.00 & 0.9968 & 0.9967 & 1.0000 & 0.9968 & 0.9972 & 1.0000 \\
 2d & k3 & p1.0 & d2.5 & 0.0275 & 99.55 & 99.48 & 99.97 & 99.59 & 99.61 & 99.94 & 0.9955 & 0.9948 & 0.9997 & 0.9959 & 0.9957 & 0.9994 \\
 2d & k3 & pinf & d1.5 & 0.0284 & 99.65 & 99.52 & 99.97 & 99.57 & 99.60 & 99.98 & 0.9965 & 0.9952 & 0.9997 & 0.9962 & 0.9959 & 0.9994 \\
 2d & k3 & p2.0 & d1.5 & 0.0296 & 99.58 & 99.32 & 99.95 & 99.63 & 99.49 & 99.93 & 0.9958 & 0.9932 & 0.9995 & 0.9966 & 0.9942 & 0.9991 \\
 2d & k3 & p2.0 & d2.5 & 0.0298 & 99.55 & 99.43 & 99.98 & 99.60 & 99.55 & 99.99 & 0.9955 & 0.9943 & 0.9998 & 0.9959 & 0.9953 & 0.9997 \\
 2d & k5 & p1.0 & d2.0 & 0.0300 & 99.42 & 99.52 & 99.92 & 99.38 & 99.57 & 99.95 & 0.9942 & 0.9952 & 0.9992 & 0.9935 & 0.9957 & 0.9985 \\
 2d & k3 & pinf & d2.5 & 0.0302 & 99.58 & 99.40 & 99.93 & 99.55 & 99.49 & 99.92 & 0.9958 & 0.9940 & 0.9993 & 0.9959 & 0.9949 & 0.9988 \\
 2d & k3 & p1.0 & d2.0 & 0.0309 & 99.52 & 99.45 & 99.97 & 99.48 & 99.59 & 99.94 & 0.9952 & 0.9945 & 0.9997 & 0.9952 & 0.9953 & 0.9994 \\
 2d & k3 & pinf & dinf & 0.0309 & 99.53 & 99.37 & 99.97 & 99.51 & 99.53 & 99.94 & 0.9953 & 0.9937 & 0.9997 & 0.9950 & 0.9946 & 0.9994 \\
 2d & k3 & p2.0 & d2.0 & 0.0313 & 99.62 & 99.40 & 99.95 & 99.61 & 99.60 & 99.93 & 0.9962 & 0.9940 & 0.9995 & 0.9965 & 0.9948 & 0.9991 \\
 2d & k3 & p1.0 & d1.5 & 0.0313 & 99.47 & 99.35 & 99.97 & 99.51 & 99.48 & 99.98 & 0.9947 & 0.9935 & 0.9997 & 0.9951 & 0.9940 & 0.9994 \\
 2d & k3 & p1.0 & dinf & 0.0321 & 99.42 & 99.50 & 99.97 & 99.41 & 99.60 & 99.98 & 0.9942 & 0.9950 & 0.9997 & 0.9932 & 0.9955 & 0.9994 \\
 2d & k5 & pinf & d2.0 & 0.0321 & 99.47 & 99.32 & 99.95 & 99.49 & 99.52 & 99.97 & 0.9947 & 0.9932 & 0.9995 & 0.9947 & 0.9941 & 0.9991 \\
 2d & k5 & pinf & d2.5 & 0.0322 & 99.52 & 99.53 & 99.98 & 99.33 & 99.68 & 99.95 & 0.9952 & 0.9953 & 0.9998 & 0.9944 & 0.9955 & 0.9997 \\
 2d & k5 & p1.0 & dinf & 0.0324 & 99.33 & 99.38 & 99.95 & 99.30 & 99.56 & 99.93 & 0.9933 & 0.9938 & 0.9995 & 0.9933 & 0.9949 & 0.9991 \\
 2d & k3 & p1.0 & d1.0 & 0.0332 & 99.53 & 99.43 & 99.93 & 99.45 & 99.61 & 99.88 & 0.9953 & 0.9943 & 0.9993 & 0.9951 & 0.9947 & 0.9988 \\
\bottomrule
\end{tabular}
